Relativistic equations for the generalized Chapman-Enskog hierarchy

From the Boltzmann equation Chapman and Cowling have firstly motivated a hierarchy of differential equations. I consider a general version of these differential equations which contain the Navier-Stokes system. In the paper I derive a relativistic version of these partial differential equations. This is interesting because in the derivation a covariant version of a time direction is used. This time direction is needed to derive a reduction of the differential equations.

==> alt-enskog.tex <==
%&latex
%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%  Chapman-Enskog hierarchy
%%  Article by Prof. H.W. Alt
%%  Copyright 2016-2016 by H. W. Alt
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% Language
\newcommand{\DE}[1]{}
\newcommand{\EN}[1]{#1}
%%
%% PDF-version
\newcommand{\PDF}[2]{#2} % in script.sty
%%
%% Nocolor
\newif\ifnocolor
\nocolortrue
%% Final version
\newif\iffinal
\finaltrue
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LaTeX-Dokument
\input{ALT-TITELEI/enskog-ltx.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




